Plug-And-Play Learned Gaussian-mixture Approximate Message Passing

Deep unfolding showed to be a very successful approach for accelerating and tuning classical signal processing algorithms. In this paper, we propose learned Gaussian-mixture AMP (L-GM-AMP) - a plug-and-play compressed sensing (CS) recovery algorithm suitable for any i.i.d. source prior. Our algorithm builds upon Borgerding's learned AMP (LAMP), yet significantly improves it by adopting a universal denoising function within the algorithm. The robust and flexible denoiser is a byproduct of modelling source prior with a Gaussian-mixture (GM), which can well approximate continuous, discrete, as well as mixture distributions. Its parameters are learned using standard backpropagation algorithm. To demonstrate robustness of the proposed algorithm, we conduct Monte-Carlo (MC) simulations for both mixture and discrete distributions. Numerical evaluation shows that the L-GM-AMP algorithm achieves state-of-the-art performance without any knowledge of the source prior.

==> figures/BG/nmse.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5.903in,
height=4.368in,
at={(0.694in,0.514in)},
scale only axis,
xmin=1,
xmax=15,
xtick={ 1,  3,  5,  7,  9, 11, 13, 15},
xlabel style={font=\color{white!15!black}},
xlabel={layer (i.e., itearation)},
ymin=-25,
ymax=0,
ylabel style={font=\color{white!15!black}},
ylabel={NMSE/dB},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, dashed, mark size=4.5pt, mark=x, mark options={solid, fill=blue, blue}]
  table[row sep=crcr]{%
1	-2.9200993\\
2	-5.409075\\
3	-7.6351304\\
4	-9.567252\\
5	-11.246672\\
6	-12.666036\\
7	-13.82929\\
8	-14.749547\\
9	-15.456907\\
10	-15.979364\\
11	-16.357471\\
12	-16.626234\\
13	-16.81567\\
14	-16.94572\\
15	-17.037313\\
16	-17.099688\\
17	-17.144926\\
18	-17.175415\\
19	-17.19807\\
20	-17.213615\\
};
\addlegendentry{AMP $\ell_1$, $N=500$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
1	-4.0697536\\
2	-7.5797844\\
3	-11.020017\\
4	-14.41029\\
5	-17.562597\\
6	-20.116814\\
7	-21.822807\\
8	-22.752766\\
9	-23.196377\\
10	-23.391745\\
11	-23.482496\\
12	-23.519812\\
13	-23.53822\\
14	-23.545639\\
15	-23.550247\\
16	-23.551645\\
17	-23.552765\\
18	-23.552706\\
19	-23.552864\\
20	-23.552544\\
};
\addlegendentry{AMP matched, $N=500$}

\addplot [color=black, dashed, mark size=4.5pt, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
1	-4.145\\
2	-7.827\\
3	-11.538\\
4	-15.289\\
5	-18.733\\
6	-21.309\\
7	-22.752\\
8	-23.38\\
9	-23.617\\
10	-23.701\\
11	-23.73\\
12	-23.741\\
13	-23.744\\
14	-23.745\\
15	-23.746\\
};
\addlegendentry{AMP matched, $N=5000$}

\addplot [color=black, draw=none, mark size=4.5pt, mark=x, mark options={solid, black}]
  table[row sep=crcr]{%
1	-4.1717773\\
2	-7.8794103\\
3	-11.635576\\
4	-15.43548\\
5	-18.901332\\
6	-21.462475\\
7	-22.855114\\
8	-23.443587\\
9	-23.663758\\
10	-23.7429333\\
};
\addlegendentry{AMP matched state evolution}

\addplot [color=mycolor1, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}]
  table[row sep=crcr]{%
1	-6.374325\\
2	-11.452974\\
3	-15.527082\\
4	-18.754254\\
5	-21.050717\\
6	-22.374766\\
};
\addlegendentry{LAMP matched, $N=500$}

\addplot [color=green, mark size=3.0pt, mark=triangle, mark options={solid, green}]
  table[row sep=crcr]{%
1	-3.689725\\
2	-11.441775\\
3	-15.599661\\
4	-18.847752\\
5	-21.091609\\
6	-22.387613\\
7	-23.013248\\
8	-23.308353\\
9	-23.404731\\
10	-23.523824\\
11	-23.562709\\
12	-23.56569\\
13	-23.567872\\
14	-23.578413\\
15	-23.578539\\
};
\addlegendentry{L-GM-AMP L=2, $N=500$}

\addplot [color=blue, mark size=7.8pt, mark=diamond, mark options={solid, blue}]
  table[row sep=crcr]{%
1	-6.488162\\
2	-11.580773\\
3	-15.690313\\
4	-18.843332\\
5	-21.11971\\
6	-22.409825\\
7	-23.0583\\
8	-23.314562\\
9	-23.434422\\
10	-23.526688\\
11	-23.550184\\
12	-23.555827\\
13	-23.565333\\
14	-23.576188\\
15	-23.569181\\
};
\addlegendentry{L-GM-AMP L=3, $N=500$}

\addplot [color=mycolor2, mark size=4.5pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
1	-6.545067\\
2	-11.547013\\
3	-15.700189\\
4	-18.759034\\
5	-20.892718\\
6	-22.159254\\
7	-22.850775\\
8	-23.210139\\
9	-23.393623\\
10	-23.47894\\
11	-23.519281\\
12	-23.533744\\
13	-23.540962\\
14	-23.546384\\
15	-23.547538\\
};
\addlegendentry{L-GM-AMP L=4, $N=500$}

\end{axis}
\end{tikzpicture}%

==> figures/Gm4_thetas/Gm4_thetas.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5.903in,
height=4.368in,
at={(0.694in,0.514in)},
scale only axis,
xmin=-1,
xmax=8,
xtick={0, 1, 2, 3, 4, 5, 6, 7, 8},
xlabel style={font=\color{white!15!black}},
xlabel={$\mu$},
ymin=-1,
ymax=5,
ylabel style={font=\color{white!15!black}},
ylabel={$\sigma^2$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, draw=none, mark size=2.0pt, mark=*, mark options={solid, fill=black, mycolor1}]
  table[row sep=crcr]{%
-0.00696479295	0.686590588\\
};
\addlegendentry{$\omega_1$ =5.35e-02}

\addplot [color=mycolor2, draw=none, mark size=14.6pt, mark=*, mark options={solid, fill=blue, mycolor2}]
  table[row sep=crcr]{%
-0.000268193965	0.000201397359\\
};
\addlegendentry{$\omega_2$ =9.14e-01}

\addplot [color=mycolor3, draw=none, mark size=5.4pt, mark=*, mark options={solid, fill=red, mycolor3}]
  table[row sep=crcr]{%
-0.0387914996	0.839766152\\
};
\addlegendentry{$\omega_3$ =1.88e-02}

\addplot [color=mycolor4, draw=none, mark size=1.5pt, mark=*, mark options={solid, fill=green, mycolor4}]
  table[row sep=crcr]{%
7.7155771	0.0186817976\\
};
\addlegendentry{$\omega_4$ =1.43e-04}

\addplot [color=mycolor5, draw=none, mark size=8.2pt, mark=o, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
-0.5	1\\
};
\addplot [color=mycolor6, draw=none, mark size=6.7pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
0.2	0.2\\
};
\addplot [color=mycolor7, draw=none, mark size=6.7pt, mark=o, mark options={solid, red}, forget plot]
  table[row sep=crcr]{%
0.5	1\\
};
\addplot [color=mycolor1, draw=none, mark size=8.2pt, mark=o, mark options={solid, green}, forget plot]
  table[row sep=crcr]{%
0.8	4\\
};
\end{axis}

\begin{axis}[%
width=6.944in,
height=5.139in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> figures/bpsk/nmse.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5.903in,
height=4.368in,
at={(0.694in,0.514in)},
scale only axis,
xmin=1,
xmax=25,
xtick={ 0,  5, 10, 15, 20, 25},
xlabel style={font=\color{white!15!black}},
xlabel={layer (i.e., itearation)},
ymin=-55,
ymax=0,
ylabel style={font=\color{white!15!black}},
ylabel={NMSE/dB},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark size=4.5pt, mark=x, mark options={solid, blue}]
  table[row sep=crcr]{%
1	-2.302\\
2	-3.6\\
3	-4.608\\
4	-5.558\\
5	-6.597\\
6	-7.888\\
7	-9.592\\
8	-11.748\\
9	-14.188\\
10	-16.67\\
11	-19.008\\
12	-21.083\\
13	-22.873\\
14	-24.466\\
15	-25.88\\
16	-27.176\\
17	-28.227\\
18	-28.986\\
19	-29.493\\
20	-29.801\\
21	-30.204\\
22	-30.551\\
23	-30.827\\
24	-30.909\\
25	-31.082\\
26	-31.201\\
27	-31.357\\
28	-31.419\\
29	-31.507\\
30	-31.571\\
};
\addlegendentry{AMP matched, $N=500$}

\addplot [color=black, mark size=4.5pt, mark=x, mark options={solid, black}]
  table[row sep=crcr]{%
1	-2.304\\
2	-3.618\\
3	-4.643\\
4	-5.616\\
5	-6.702\\
6	-8.118\\
7	-10.306\\
8	-14.306\\
9	-22.084\\
10	-34.877\\
11	-48.444\\
12	-50.17\\
13	-50.211\\
14	-50.145\\
15	-50.191\\
16	-50.151\\
17	-50.191\\
18	-50.154\\
19	-50.193\\
20	-50.156\\
21	-50.195\\
22	-50.156\\
23	-50.197\\
24	-50.156\\
25	-50.199\\
26	-50.156\\
27	-50.2\\
28	-50.156\\
29	-50.201\\
30	-50.156\\
};
\addlegendentry{AMP matched, $N=5000$}

\addplot [color=black, mark size=4.5pt, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
1	-2.24370163817752\\
2	-3.57823667925829\\
3	-4.81525086870251\\
4	-5.96195509298597\\
5	-7.17186350454994\\
6	-8.9628614933805\\
7	-12.0606925323085\\
8	-19.276884687131\\
9	-38.6426820499865\\
10	-124.264724476404\\
};
\addlegendentry{AMP matched state evolution}

\addplot [color=mycolor1, mark size=3.2pt, mark=square, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
1	-3.975\\
2	-4.754\\
3	-6.346\\
4	-7.637\\
5	-10.04\\
6	-12.961\\
7	-16.481\\
8	-20.374\\
9	-23.625\\
10	-26.455\\
11	-28.531\\
12	-30.531\\
13	-32.056\\
14	-32.935\\
15	-33.628\\
16	-33.612\\
17	-33.636\\
18	-33.505\\
19	-34.483\\
20	-34.379\\
21	-34.748\\
22	-34.733\\
23	-34.821\\
24	-36.25\\
25	-35.782\\
};
\addlegendentry{L-GM-AMP L=4, $N=500$}

\end{axis}
\end{tikzpicture}%

==> figures/dm/nmse.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{mycolor2}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor3}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5.903in,
height=4.368in,
at={(0.694in,0.514in)},
scale only axis,
xmin=1,
xmax=15,
xtick={ 1,  3,  5,  7,  9, 11, 13, 15},
xlabel style={font=\color{white!15!black}},
xlabel={layer (i.e., itearation)},
ymin=-40,
ymax=0,
ylabel style={font=\color{white!15!black}},
ylabel={NMSE/dB},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1	-1.933\\
2	-3.177\\
3	-4.357\\
4	-5.732\\
5	-7.395\\
6	-9.181\\
7	-10.886\\
8	-12.388\\
9	-13.689\\
10	-14.767\\
11	-15.67\\
12	-16.432\\
13	-17.064\\
14	-17.594\\
15	-18.08\\
16	-18.472\\
17	-18.835\\
18	-19.14\\
19	-19.42\\
20	-19.61\\
21	-19.769\\
22	-19.908\\
23	-20.051\\
24	-20.154\\
25	-20.26\\
26	-20.334\\
27	-20.43\\
28	-20.474\\
29	-20.541\\
30	-20.574\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	-2.505\\
2	-4.702\\
3	-7.74\\
4	-12.455\\
5	-18.397\\
6	-24.388\\
7	-29.727\\
8	-34.534\\
9	-39.507\\
10	-44.977\\
11	-46.996\\
12	-51.645\\
};
\addplot [color=blue, draw=none, mark size=4.5pt, mark=x, mark options={solid, blue}]
  table[row sep=crcr]{%
1	-1.933\\
2	-3.177\\
3	-4.357\\
4	-5.732\\
5	-7.395\\
6	-9.181\\
7	-10.886\\
8	-12.388\\
9	-13.689\\
10	-14.767\\
11	-15.67\\
12	-16.432\\
13	-17.064\\
14	-17.594\\
15	-18.08\\
16	-18.472\\
17	-18.835\\
18	-19.14\\
19	-19.42\\
20	-19.61\\
21	-19.769\\
22	-19.908\\
23	-20.051\\
24	-20.154\\
25	-20.26\\
26	-20.334\\
27	-20.43\\
28	-20.474\\
29	-20.541\\
30	-20.574\\
};
\addlegendentry{AMP matched}

\addplot [color=mycolor1, draw=none, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}]
  table[row sep=crcr]{%
1	-2.209182\\
2	-3.86051\\
3	-5.5609\\
4	-8.05939\\
5	-10.752326\\
6	-13.110082\\
7	-15.199554\\
8	-16.855165\\
9	-18.178262\\
10	-19.310715\\
11	-20.220153\\
12	-20.822711\\
13	-21.413711\\
14	-21.94974\\
15	-22.410865\\
};
\addlegendentry{LAMP matched}

\addplot [color=mycolor2, draw=none, mark size=4.5pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
1	-3.173701\\
2	-5.233571\\
3	-7.555081\\
4	-10.184839\\
5	-12.692851\\
6	-14.899814\\
7	-16.828593\\
8	-18.215848\\
9	-19.383713\\
10	-20.190838\\
11	-20.969333\\
12	-21.561835\\
13	-22.18957\\
14	-22.461876\\
15	-22.612928\\
};
\addlegendentry{L-GM-AMP L=4}

\addplot [color=blue, mark size=4.5pt, mark=x, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1	-1.933\\
2	-3.177\\
3	-4.357\\
4	-5.732\\
5	-7.395\\
6	-9.181\\
7	-10.886\\
8	-12.388\\
9	-13.689\\
10	-14.767\\
11	-15.67\\
12	-16.432\\
13	-17.064\\
14	-17.594\\
15	-18.08\\
16	-18.472\\
17	-18.835\\
18	-19.14\\
19	-19.42\\
20	-19.61\\
21	-19.769\\
22	-19.908\\
23	-20.051\\
24	-20.154\\
25	-20.26\\
26	-20.334\\
27	-20.43\\
28	-20.474\\
29	-20.541\\
30	-20.574\\
};
\addplot [color=mycolor1, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}, forget plot]
  table[row sep=crcr]{%
1	-2.209182\\
2	-3.86051\\
3	-5.5609\\
4	-8.05939\\
5	-10.752326\\
6	-13.110082\\
7	-15.199554\\
8	-16.855165\\
9	-18.178262\\
10	-19.310715\\
11	-20.220153\\
12	-20.822711\\
13	-21.413711\\
14	-21.94974\\
15	-22.410865\\
};
\addplot [color=mycolor3, mark size=4.5pt, mark=o, mark options={solid, mycolor3}, forget plot]
  table[row sep=crcr]{%
1	-3.173701\\
2	-5.233571\\
3	-7.555081\\
4	-10.184839\\
5	-12.692851\\
6	-14.899814\\
7	-16.828593\\
8	-18.215848\\
9	-19.383713\\
10	-20.190838\\
11	-20.969333\\
12	-21.561835\\
13	-22.18957\\
14	-22.461876\\
15	-22.612928\\
};
\addplot [color=blue, dashed, mark size=4.5pt, mark=x, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1	-2.505\\
2	-4.702\\
3	-7.74\\
4	-12.455\\
5	-18.397\\
6	-24.388\\
7	-29.727\\
8	-34.534\\
9	-39.507\\
10	-44.977\\
11	-46.996\\
12	-51.645\\
};
\addplot [color=mycolor1, dashed, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}, forget plot]
  table[row sep=crcr]{%
1	-3.18254\\
2	-6.665087\\
3	-13.218741\\
4	-23.771548\\
5	-34.013941\\
6	-41.562875\\
7	-49.411778\\
};
\addplot [color=mycolor3, dashed, mark size=4.5pt, mark=o, mark options={solid, mycolor3}, forget plot]
  table[row sep=crcr]{%
1	-4.511\\
2	-10.084\\
3	-17.982\\
4	-26.717\\
5	-33.44\\
6	-40.586\\
7	-46.486\\
};
\end{axis}
\end{tikzpicture}%

==> figures/dm/ser.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.722in,
height=4.368in,
at={(0.556in,0.514in)},
scale only axis,
xmin=1,
xmax=15,
xtick={ 1,  3,  5,  7,  9, 11, 13, 15},
xlabel style={font=\color{white!15!black}},
xlabel={layer (i.e., itearation)},
ymode=log,
ymin=1e-05,
ymax=0.2,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={symbol error rate},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=black, forget plot]
  table[row sep=crcr]{%
1	0.0811832\\
2	0.0622698\\
3	0.0476858\\
4	0.034735\\
5	0.0236412\\
6	0.0156676\\
7	0.0105752\\
8	0.007471\\
9	0.0055384\\
10	0.0043052\\
11	0.003486\\
12	0.0029372\\
13	0.002536\\
14	0.002243\\
15	0.0019968\\
16	0.0018122\\
17	0.0016756\\
18	0.001553\\
19	0.0014544\\
20	0.0013946\\
};
\addplot [color=black, dashed, forget plot]
  table[row sep=crcr]{%
1	0.0721206\\
2	0.0441536\\
3	0.0219348\\
4	0.0073792\\
5	0.0018664\\
6	0.0004674\\
7	0.0001382\\
8	4.44e-05\\
9	1.46e-05\\
10	3.2e-06\\
11	2.2e-06\\
12	8e-07\\
};
\addplot [color=blue, draw=none, mark size=4.5pt, mark=x, mark options={solid, blue}]
  table[row sep=crcr]{%
1	0.0811832\\
2	0.0622698\\
3	0.0476858\\
4	0.034735\\
5	0.0236412\\
6	0.0156676\\
7	0.0105752\\
8	0.007471\\
9	0.0055384\\
10	0.0043052\\
11	0.003486\\
12	0.0029372\\
13	0.002536\\
14	0.002243\\
15	0.0019968\\
16	0.0018122\\
17	0.0016756\\
18	0.001553\\
19	0.0014544\\
20	0.0013946\\
};
\addlegendentry{AMP matched}

\addplot [color=mycolor1, draw=none, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}]
  table[row sep=crcr]{%
1	0.0797164\\
2	0.044175\\
3	0.032577\\
4	0.0208758\\
5	0.0112106\\
6	0.0066748\\
7	0.004267\\
8	0.002989\\
9	0.00227\\
10	0.0017964\\
11	0.0014896\\
12	0.0013\\
13	0.0011502\\
14	0.0010356\\
15	0.0009328\\
};
\addlegendentry{LAMP matched}

\addplot [color=mycolor2, draw=none, mark size=4.5pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
1	0.103781\\
2	0.0827618\\
3	0.0370012\\
4	0.0223728\\
5	0.0129388\\
6	0.0073808\\
7	0.0043598\\
8	0.0028872\\
9	0.0020228\\
10	0.0015878\\
11	0.0012962\\
12	0.0011586\\
13	0.0010194\\
14	0.000953\\
15	0.0008836\\
};
\addlegendentry{L-GM-AMP L=4}

\addplot [color=blue, mark size=4.5pt, mark=x, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1	0.0811832\\
2	0.0622698\\
3	0.0476858\\
4	0.034735\\
5	0.0236412\\
6	0.0156676\\
7	0.0105752\\
8	0.007471\\
9	0.0055384\\
10	0.0043052\\
11	0.003486\\
12	0.0029372\\
13	0.002536\\
14	0.002243\\
15	0.0019968\\
16	0.0018122\\
17	0.0016756\\
18	0.001553\\
19	0.0014544\\
20	0.0013946\\
};
\addplot [color=mycolor1, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}, forget plot]
  table[row sep=crcr]{%
1	0.0797164\\
2	0.044175\\
3	0.032577\\
4	0.0208758\\
5	0.0112106\\
6	0.0066748\\
7	0.004267\\
8	0.002989\\
9	0.00227\\
10	0.0017964\\
11	0.0014896\\
12	0.0013\\
13	0.0011502\\
14	0.0010356\\
15	0.0009328\\
};
\addplot [color=mycolor2, mark size=4.5pt, mark=o, mark options={solid, mycolor2}, forget plot]
  table[row sep=crcr]{%
1	0.103781\\
2	0.0827618\\
3	0.0370012\\
4	0.0223728\\
5	0.0129388\\
6	0.0073808\\
7	0.0043598\\
8	0.0028872\\
9	0.0020228\\
10	0.0015878\\
11	0.0012962\\
12	0.0011586\\
13	0.0010194\\
14	0.000953\\
15	0.0008836\\
};
\addplot [color=blue, dashed, mark size=4.5pt, mark=x, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1	0.0721206\\
2	0.0441536\\
3	0.0219348\\
4	0.0073792\\
5	0.0018664\\
6	0.0004674\\
7	0.0001382\\
8	4.44e-05\\
9	1.46e-05\\
10	3.2e-06\\
11	2.2e-06\\
12	8e-07\\
};
\addplot [color=mycolor1, dashed, mark size=3.0pt, mark=triangle, mark options={solid, rotate=180, mycolor1}, forget plot]
  table[row sep=crcr]{%
1	0.0567106\\
2	0.0189064\\
3	0.0049248\\
4	0.000528\\
5	4.84e-05\\
6	6.2e-06\\
7	1.4e-06\\
};
\addplot [color=mycolor2, dashed, mark size=4.5pt, mark=o, mark options={solid, mycolor2}, forget plot]
  table[row sep=crcr]{%
1	0.0440888\\
2	0.0174738\\
3	0.0044442\\
4	0.0004796\\
5	5.04e-05\\
6	9e-06\\
};
\end{axis}
\end{tikzpicture}%
